LWE with Quantum Amplitudes: Algorithm, Hardness, and Oblivious Sampling

In this paper, we show new algorithms, hardness results and applications for $\sf{S|LWE\rangle}$ and $\sf{C|LWE\rangle}$ with real Gaussian, Gaussian with linear or quadratic phase terms, and other related amplitudes. Let $n$ be the dimension of LWE samples. Our main results are 1. There is a $2^{\tilde{O}(\sqrt{n})}$-time algorithm for $\sf{S|LWE\rangle}$ with Gaussian amplitude with \emph{known} phase, given $2^{\tilde{O}(\sqrt{n})}$ many quantum samples. The algorithm is modified from Kuperberg's sieve, and in fact works for more general amplitudes as long as the amplitudes and phases are completely \emph{known}. 2. There is a polynomial time quantum algorithm for solving $\sf{S|LWE\rangle}$ and $\sf{C|LWE\rangle}$ for Gaussian with quadratic phase amplitudes, where the sample complexity is as small as $\tilde{O}(n)$. As an application, we give a quantum oblivious LWE sampler where the core quantum sampler requires only quasi-linear sample complexity. This improves upon the previous oblivious LWE sampler given by Debris-Alazard, Fallahpour, Stehl\'{e} [STOC 2024], whose core quantum sampler requires $\tilde{O}(nr)$ sample complexity, where $r$ is the standard deviation of the error. 3. There exist polynomial time quantum reductions from standard LWE or worst-case GapSVP to $\sf{S|LWE\rangle}$ with Gaussian amplitude with small \emph{unknown} phase, and arbitrarily many samples. Compared to the first two items, the appearance of the unknown phase term places a barrier in designing efficient quantum algorithm for solving standard LWE via $\sf{S|LWE\rangle}$.

==> rebuttal.tex <==
\section{Rebuttal}

We thank reviewers for their helpful comments.

A common question: how to interpret our quantum reductions from GapSVP/LWE to S|LWE> with unknown phases?

Chen, Liu, and Zhandry show that S|LWE> whose error amplitude is known with wide DFT is solvable, Brakerski et al. show that EDCP (which is equivalent to S|LWE>) with polynomial many samples is as hard as LWE. The hardness of S|LWE> when the number is super-polynomial and the error amplitude is Gaussian-like, remains largely unexplored. Our work, to a certain degree, fills the blank in both hardness and algorithm directions.

However, we want to point out that, the main motivation of presenting those reductions is to illustrate new approaches of designing quantum algorithms for solving standard LWE. Our results show that one possibility of solving standard LWE is to quantumly solving S|LWE> with unknown phase (but we know the phase is relatively small compared to the modulus and also the distribution is known).

For reviewer B: we would like to clarify that we did not intend to downplay the importance of the unknown phase (we apologize if we gave you the impression that the unknown phase is a minor issue). On the contrary, whether the presence of the unknown phase is an "inherent" obstacle or a "hopefully solvable" obstacle is debatable.

% we apologize that we gave you an impression that the unknown phase is a small obstacle. We have to emphasize that, we didn't want to give such an impression. What's more, whether the presence of the unknown phase is an "inherent" obstacle or a "hopefully solvable" obstacle is debatable. 

%You are wondering if our approach has no advantage compared to previous approaches. We want to heuristically give you an impression that our approach has some advantages: 

You are wondering if the unknown phase will lead to a classical LWE sample. We would like to highlight that although the phase is not easy to compute, there is still some hope to utilize the phase to design subexponential algorithms for S|LWE> with unknown phase.
In fact, we have tried some ways of extracting (or approximating) the unknown phase. For example, for the reduction presented in Section 3, we have tried to use the ``filtering'' technique from CLZ22 to guess the phase. Another way that we tried is to use Kuperberg sieve on both $a$ and the measured out information $y$ (which determines the phase). Unfortunately, those attempts fail due to subtle reasons, so we didn't discuss them in the paper. But maybe we can add a discussion on the possibilities of utilizing the phase. We hope that this work will inspire researchers to pay more attention to the unknown phase, and finally come up with innovative ways of utilizing the unknown phase to solve the problem.

Furthermore, you have said that "BKSW cannot run Kuperberg because of their inverse polynomial error, but once you assume away this error, there is no barrier." We have to point out that the inverse polynomial error in BKSW is a substantial obstacle, and whether an EDCP state is generated with error is not detectable. So one cannot easily assume away this error to run Kuperberg sieve.

% To summarize, we think the reductions from GapSVP/LWE to S|LWE> with unknown phases give another hope of trying to design quantum algorithms for solving lattice problems. The obstacle presented by the unknown phase is substantial (we will update the paper to reflect this point), but there might be a hope of using some new quantum techniques to overcome it.


Reviewer A's Q1: On page 21, why do you measure the first register to get a state close to $\gamma_t^a$ at step 5?

A: We guess Reviewer A asked this question because in Section 4.4, we didn't measure the first register $|y>$. Indeed, on page 21, we measure the first register only for a better illustration of the residual state. 

Q2: While Chen, Liu, and Zhandry show that S|LWE> whose error amplitude is known with wide DFT, this work shows that S|LWE> whose error amplitude is Gaussian with unknown phase is as hard as LWE.
I still need to get what those results mean for the (quantum) hardness of LWE.
Could you explain an interpretation of those results? What observations can we get from those?

A: Those results show that there are several possibilities of quantumly solving standard LWE by further improving the quantum algorithms for solving S|LWE>. For the CLZ result, if we can further reduce the number of samples, then great. For the result in the current submission, if we can handle the unknown phase, then there is a chance of getting subexponential time quantum algorithm for solving LWE.



Reviewer C's Q1: Can you please add some discussion on the differences between the reduction from GapSVP to $SLWE^{phase}$ obtained from sections 3 and 4?

A: Let us explain the differences from two angles. 1. The quality of the reductions (the reduction from section 3 works when $q = \widetilde{\Omega}(n^2)$ while the reduction from section 4 works when $q = \Omega(n)$). 
2. Differences in the reduction algorithms, so if someone wants to make improvements, the two algorithms provide different options. The algorithm in section 3 is easier to start with when thinking about improvements (e.g. by guessing the phase).

Q2: What are the main differences between the LWE-EDCP reduction from section 3 and from Brakerski et al.'s? Is it mainly a tradeoff between number of samples and having to introduce unknown centers in the distribution?

A: Exactly a tradeoff. Our main motivation is to create unbounded number of samples. As we have shown, if we have sub-exponentially many samples without phase or with known phase, there exists sub-exponential time quantum algorithm. The main obstacle of Brakerski et al.'s reduction is the inverse polynomial fail probability that avoids producing sub-exponential many samples, and this obstacle is hard to address. We overcome this obstacle, while introducing an unknown phase on the S|LWE> states.

==> rebuttal_crypto.tex <==
We thank reviewers for their helpful comments.

- Reply to Reviewer A

We agree that a collapsed state is not interesting, and therefore, we need to be careful whether the S|LWE>phase collapses to LWE for our phase function. However, we would like to point out that

1. As Reviewer A already noticed, $\rho := \sum_y \Psi_y\Psi_y^\dagger$ is collapsed for many choices of the phase function. Thus we cannot hope to get a non-trivial algorithm if we ignore the $y$ register (we also observed this, see Remark 7). However, after taking the $y$ register into consideration as we did in the Definition 3, for the phase function $\theta(y) := y/q$, the state can be written as $\rho' := \sum_y \Psi_y\Psi_y^\dagger \otimes \ketbra{y}{y}$, which is clearly not collapsed as we can apply a unitary to it to get $ \Psi_0\Psi_0^\dagger \otimes \sum_y\ketbra{y}{y}$ (and actually our subexponential algorithm in Section 5 applies to this state $\Psi_0\Psi_0^\dagger$).

2. Another reason that our phase function may be interesting: the Gaussian distribution assigns more weight on short vectors than a uniform distribution. As discussed in Remark 5, in our S|LWE>phase instance, the phase has relatively small absolute value with almost certainty. We believe it is non-trivial and may be potentially utilized. (On the one extreme where the phase goes to zero, our algorithm in Section 5 works to solve the corresponding S|LWE>phase problem. )

---
About definition 3: 
* The domain of $f$ may contain non-integer points (as in Section 4). It can be in general viewed as a subset of $\{e \in \R: -q/2 < e \leq q/2\}$. 
* $e$ is interpreted as a real number such that $-q/2 < e \leq q/2$.

---
About theorem 5:
We thank Reviewer A for pointing out this inappropriate expression. We say that a quantum algorithm can solve S|LWE>phase in the following sense (The definition of ``that can solve'' is defined in definition 3): the quantum algorithm is given samples of any S|LWE>phase problem (with any hidden secret vector $s$) from the class of parameterized S|LWE>phase problems with all $E \in \{1, 2, \cdots, \gamma^2 m\}$ and **all $e$ such that $\|e\| \leq \gamma \sqrt{m}$**, and outputs the secret vector with probability $1 - 2^{-\Omega(n)}$. 

The correct formulation of our statement is:  Suppose there exists a quantum algorithm that can solve S|LWE>phase in the above sense with $\ell = 2^{o(n)}$ samples in time $T = 2^{o(n)}$, then there exists a quantum algorithm such that given the LWE instance with any secret vector $s$, can output the $s$ with probability $1 - 2^{-\Omega(n)}$ in time $O((T + \ell \cdot \poly(n, q)) \cdot \gamma^2m)$.

- Reply to Reviewer C

(Reply to the comparison of Gaussian standard deviation between ours and [BKSW18].)

Comparison of Gaussian standard deviation between our Theorem 3 and [BKSW18]: 
Given an LWE sample with noise ratio alpha (st. dev. alpha * q) where m = Theta (n log q), [BKSW18] roughly reduces it into the problem of solving |EDCP> given l samples with st. dev. r <= 1 / (l * alpha * poly).

Given an LWE sample with noise ratio gamma' = gamma / q (st. dev. gamma) where m = Theta(n log q), Theorem 3 reduces it into the problem of solving |EDCP> given $l = 2^{o(n)}$ samples with st. dev. sigma = Theta(alpha), which can be as small as roughly sqrt(n), and can be as large as q / (16 m gamma sqrt(log q)) = 1/ (gamma' * poly) with the cost of introducing some unknown center c. This also explains the interplay between our parameters gamma and alpha in Theorem 3.

Thus the st. dev. in our reduction can be larger when we want super-polynomial |EDCP> samples.

We understand that Reviewer C may expect an answer to the question like "does our reduction reduce LWE with smaller modulus-noise ratio (q/gamma) to an EDCP-like problem, compared to BKSW18"? We would like to point out that both our paper and BKSW18 provide results with tradeoffs in parameters, in particular, different q/gamma leads to qualitatively different EDCP instances, so strictly speaking the two results are incomparable. 

(Reply to 'In the proof of Thm.3: why not to use Minkowski-Hlawka for a (probabilistic) lower bound on lambda\_1?'.)

---
About the lower bound on lambda\_1: 
Minkowski-Hlawka will give a bound, but we choose to follow the proof idea in [GPV08] as it is more straightforward and might give a tighter bound than Minkowski-Hlawka.

% (Reply to 'interplay between $\alpha$ and $\gamma$ in theorem 3'.)

---
About step 2 of theorem 15: 
We agree that having an efficient identification of the two points is crucial. Theorem 15 is stated under the 'existence of an efficient algorithm that finds the desired pair of points', which usually holds when we consider the typical error distribution (amplitude) is Gaussian or bounded uniform distribution. Moreover, if $q$ is polynomial (or sub-exponential) in $n$ then the DFT of the amplitude function $f$ can be computed in polynomial (or sub-exponential) time classically as long as $f$ is completely known, and so are the desired pair of points. 

---
We thank Reviewer C for pointing out the inconsistency and ambiguity in our notations. We'll unify the subindices to the same meaning in a future version. 
